Probing the nature of dark energy through galaxy redshift surveys with radio telescopes

Galaxy redshift surveys using optical telescopes have, in combination with other cosmological probes, enabled precision measurements of the nature of dark energy. We show that radio telescopes are rapidly becoming competitive with optical facilities in spectroscopic surveys of large numbers of galaxies. Two breakthroughs are driving this change. Firstly, individual radio telescopes are more efficient at mapping the sky thanks to the large field-of-view of new phased-array feeds. Secondly, ever more dishes can be correlated in a cost-effective manner with rapid increases in computing power. The next decade will see the coming of age of the 21cm radio wavelength as a cosmological probe as first the Pathfinders then, ultimately, the Square Kilometre Array is constructed. The latter will determine precise 3D positions for a billion galaxies, mapping the distribution of matter in the Universe over the last 12 billion years. This radio telescope will be able to constrain the equation of state of dark energy, and its potential evolution, to a precision rivalling that of future optical facilities such as DESI and Euclid.

==> HI_Pk_Review arxiv/jdefs.tex <==
% bibliography and bibfile journal definitions (taken from aa.cls)

\def\aj{AJ}					% Astronomical Journal
\def\araa{ARA\&A}				% Annual Review of Astron and Astrophys
\def\apj{ApJ}					% Astrophysical Journal
\def\apjl{ApJL}					% Astrophysical Journal, Letters
\def\apjs{ApJS}					% Astrophysical Journal, Supplement
\def\ao{Appl.~Opt.}				% Applied Optics
\def\apss{Ap\&SS}				% Astrophysics and Space Science
\def\aap{A\&A}					% Astronomy and Astrophysics
\def\aapr{A\&A~Rev.}				% Astronomy and Astrophysics Reviews
\def\aaps{A\&AS}				% Astronomy and Astrophysics, Supplement
\def\azh{AZh}					% Astronomicheskii Zhurnal
\def\baas{BAAS}					% Bulletin of the AAS
\def\jrasc{JRASC}				% Journal of the RAS of Canada
\def\memras{MmRAS}				% Memoirs of the RAS
\def\mnras{MNRAS}				% Monthly Notices of the RAS
\def\pra{Phys.~Rev.~A}				% Physical Review A: General Physics
\def\prb{Phys.~Rev.~B}				% Physical Review B: Solid State
\def\prc{Phys.~Rev.~C}				% Physical Review C
\def\prd{Phys.~Rev.~D}				% Physical Review D
\def\pre{Phys.~Rev.~E}				% Physical Review E
\def\prl{Phys.~Rev.~Lett.}			% Physical Review Letters
\def\pasp{PASP}					% Publications of the ASP
\def\pasj{PASJ}					% Publications of the ASJ
\def\qjras{QJRAS}				% Quarterly Journal of the RAS
\def\skytel{S\&T}				% Sky and Telescope
\def\solphys{Sol.~Phys.}			% Solar Physics
\def\sovast{Soviet~Ast.}			% Soviet Astronomy
\def\ssr{Space~Sci.~Rev.}			% Space Science Reviews
\def\zap{ZAp}					% Zeitschrift fuer Astrophysik
\def\nat{Nature}				% Nature
\def\iaucirc{IAU~Circ.}				% IAU Cirulars
\def\aplett{Astrophys.~Lett.}			% Astrophysics Letters
\def\apspr{Astrophys.~Space~Phys.~Res.}		% Astrophysics Space Physics Research
\def\bain{Bull.~Astron.~Inst.~Netherlands}	% Bulletin Astronomical Institute of the Netherlands
\def\fcp{Fund.~Cosmic~Phys.}			% Fundamental Cosmic Physics
\def\gca{Geochim.~Cosmochim.~Acta}		% Geochimica Cosmochimica Acta
\def\grl{Geophys.~Res.~Lett.}			% Geophysics Research Letters
\def\jcp{J.~Chem.~Phys.}			% Journal of Chemical Physics
\def\jcap{JCAP}			% Journal of Cosmology and Astroparticle Physics
\def\jgr{J.~Geophys.~Res.}			% Journal of Geophysics Research
\def\jqsrt{J.~Quant.~Spec.~Radiat.~Transf.}	% Journal of Quantitiative Spectroscopy and Radiative Trasfer
\def\memsai{Mem.~Soc.~Astron.~Italiana}		% Mem. Societa Astronomica Italiana
\def\nar{NAR}			% New Astronomy Reviews
\def\nphysa{Nucl.~Phys.~A}			% Nuclear Physics A
\def\pasa{PASA}			% Physics Reports
\def\physrep{Phys.~Rep.}			% Physics Reports
\def\physscr{Phys.~Scr}				% Physica Scripta
\def\planss{Planet.~Space~Sci.}			% Planetary Space Science
\def\procspie{Proc.~SPIE}			% Proceedings of the SPIE
\let\astap=\aap
\let\apjlett=\apjl
\let\apjsupp=\apjs
\let\applopt=\ao

% end of file


